Ray-Patch: An Efficient Querying for Light Field Transformers

In this paper we propose the Ray-Patch querying, a novel model to efficiently query transformers to decode implicit representations into target views. Our Ray-Patch decoding reduces the computational footprint and increases inference speed up to one order of magnitude compared to previous models, without losing global attention, and hence maintaining specific task metrics. The key idea of our novel querying is to split the target image into a set of patches, then querying the transformer for each patch to extract a set of feature vectors, which are finally decoded into the target image using convolutional layers. Our experimental results, implementing Ray-Patch in 3 different architectures and evaluating it in 2 different tasks and datasets, demonstrate and quantify the effectiveness of our method, specifically a notable boost in rendering speed for the same task metrics.

==> figures/tex_fps_vs_resolution.tex <==
\begin{figure*}[t]
  %\hspace*{-1cm}
\begin{subfigure}{0.49\linewidth}
\begin{tikzpicture}
\centering
  \begin{axis}[
      myplotstyle,
      legend pos=north west,
      legend entries={{DeFiNe}, {RP k=4}, {RP k=8}, {RP k=16}, {RP k=32}},
      %legend style={anchor=north west, at={(0.0,1.15)},legend columns=-1},
      ylabel={vRAM (GBytes)},
      xlabel={Resolution},
      xtick=data,
      xticklabels={128x192, 240x320, 480x640, 960x1280},
      xmode=log,
      width = 0.98\linewidth,
      height = 0.9\linewidth,
      cycle list name=exotic,
  ]  
  \addplot+[] table[x=RAM,y=define, col sep=comma]  {figures/RAMvsRES_define.csv};
  \addplot+[cyan!60!black,mark options={fill=cyan!80!black}] table[x=RAM,y=rp_define_k4, col sep=comma]  {figures/RAMvsRES_define.csv};
  \addplot+[red!70!white,mark=star, mark options={fill=red!70!white}] table[x=RAM,y=rp_define_k8, col sep=comma]  {figures/RAMvsRES_define.csv};
  \addplot+[lime!80!black, mark=diamond, mark options={fill=lime}] table[x=RAM,y=rp_define_k16, col sep=comma]  {figures/RAMvsRES_define.csv};
  %\addplot+[red, mark=*, mark options={solid, fill=red!80!black}] table[x=RAM,y=rp_define_k32, col sep=comma]  {figures/RAMvsRES_define.csv};
  \end{axis}
\end{tikzpicture}
\caption{}
\label{fig:ramVsRes_define}
\end{subfigure}
\begin{subfigure}{0.49\linewidth}
\vspace{-20cm}
\begin{tikzpicture}
\centering
  \begin{axis}[
      myplotstyle,
      legend pos=north east,
      legend entries={{DeFiNe}, {RP k=4}, {RP k=8}, {RP k=16}, {RP k=32}},
      legend style={only marks,anchor=north west, at={(0.0,1.10)},legend columns=-1},
      ylabel={FPS},
      xlabel={Resolution},
      xtick=data,
      xticklabels={128x192, 240x320, 480x640, 960x1280},
      xmode=log,
      width = 0.98\linewidth,
      height = 0.9\linewidth,
      cycle list name=exotic,
  ]  
  \addplot+[] table[x=resolution,y=define, col sep=comma]  {figures/FPS_vs_resolution.csv};
  \addplot+[cyan!60!black,mark options={fill=cyan!80!black}] table[x=resolution,y=rp_define_k4, col sep=comma]  {figures/FPS_vs_resolution.csv};
  \addplot+[red!70!white,mark=star, mark options={fill=red!70!white}] table[x=resolution,y=rp_define_k8, col sep=comma]  {figures/FPS_vs_resolution.csv};
  \addplot+[lime!80!black, mark=diamond, mark options={fill=lime}] table[x=resolution,y=rp_define_k16, col sep=comma]  {figures/FPS_vs_resolution.csv};
  %\addplot+[red, mark=*, mark options={solid, fill=red!80!black}] table[x=resolution,y=rp_define_k32, col sep=comma]  {figures/FPS_vs_resolution.csv};
  \end{axis}
\end{tikzpicture}
\caption{}
\label{fig:fpsres}
\end{subfigure}
\caption{\textit{(a)} \textbf{Peak GPU vRAM usage due to attention} for decoding a single image. vRAM usage scales linearly with the number of pixels (quadratically with resolution). Ray-Patch querying reduces \(\times10\) required resources on standard resolutions. Note that $x$-axis is in logarithmic scale. \textit{(b)} \textbf{Single image rendering speed scaling.} The use of the Ray-Patch decoder increase rendering speed at high resolutions up to real-time for DeFiNe. To keep a fixed rendering speed, the patch size should increase at the same pace as the number of pixels.}
\end{figure*}

==> figures/tex_scannet.tex <==
\begin{figure*}
    \centering
    \newcommand\y{200} %For two input samples, image306
    %\newcommand\y{136}
    \begin{picture}(\linewidth,\y)(0,0)
    \put(0,0){\includegraphics[width=\linewidth]{figures/scannet2.png}}
    \put(27, \numexpr\y-9){\fontsize{12}{0}\selectfont Input}
    \put(00, \numexpr\y-13){ \line(1, 0){78} }
    \put(107, \numexpr\y-9){\fontsize{12}{0}\selectfont DeFiNe}
    \put(82, \numexpr\y-13){ \line(1, 0){78} }
    
    \put(180, \numexpr\y-9){\fontsize{12}{0}\selectfont RP-DeFiNe}
    \put(165, \numexpr\y-13){ \line(1, 0){78} }
    
    \put(273, \numexpr\y-9){\fontsize{12}{0}\selectfont Target}
    \put(249, \numexpr\y-13){ \line(1, 0){77} }
    \put(352, \numexpr\y-9){\fontsize{12}{0}\selectfont DeFiNe}
    \put(331, \numexpr\y-13){ \line(1, 0){77} }
    \put(424, \numexpr\y-9){\fontsize{12}{0}\selectfont RP-DeFiNe}
    \put(415, \numexpr\y-13){ \line(1, 0){77} }
    
    \end{picture}
    
    \caption{Novel View Synthesis comparison}
    \label{fig:scannet}
\end{figure*}

